ASR data augmentation in low-resource settings using cross-lingual multi-speaker TTS and cross-lingual voice conversion

We explore cross-lingual multi-speaker speech synthesis and cross-lingual voice conversion applied to data augmentation for automatic speech recognition (ASR) systems in low/medium-resource scenarios. Through extensive experiments, we show that our approach permits the application of speech synthesis and voice conversion to improve ASR systems using only one target-language speaker during model training. We also managed to close the gap between ASR models trained with synthesized versus human speech compared to other works that use many speakers. Finally, we show that it is possible to obtain promising ASR training results with our data augmentation method using only a single real speaker in a target language.

==> reviews.tex <==
Reviewer #4
Questions
1. Reviewer confidence (1-3) By selecting a value, you confirm that you are competent to evaluate this paper. If you have doubts about your ability to assess it, do not complete this form but instead use "Contact Meta-Reviewer". 
2: Confident
2. Technical correctness of the work (1-4) Please evaluate the scientific and/or technical correctness of the work. If experiments are presented please consider if enough details are provided on the datasets, baseline and experimental design to allow the experiments to be reproduced or equivalent experiments run. If you give a score of 1 or 2, please provide further explanation in your Detailed Comments.
3: Minor issues but credible results
3. Clarity of presentation Please evaluate the clarity of the presentation of the work. Take into account the writing and quality of figures, tables etc. If you give a score of 1 or 2 please provide further explanation in your Detailed Comments.
3. Clear enough, could benefit from some revision
4. Overall recommendation (1-6)
4: Weak Accept: I am leaning to accept this paper
5. Detailed Comments for Authors Please supply detailed comments to back up your rankings. These comments will be forwarded to the authors of the paper. The comments will help the committee decide the outcome of the paper, and will help justify this decision for the authors. If the paper is accepted, the comments should guide the authors in making revisions for a final manuscript. Hence, the more detailed you make your comments, the more useful your review will be - both for the committee and for the authors. (min. 120 words). Particularly, provide feedback on the following topics: * Key Strength of the paper * Main Weakness of the paper * Novelty/Originality, taking into account the relevance of the work for the Interspeech audience * Technical Correctness, is the work technically and/or scientifically solid? Are sufficient details provided to allow any experiments to be reproduced or equivalent experiments run? * Quality of References, is it a good mix of older and newer papers? Do the authors show a good grasp of the current state of the literature? Do they also cite other papers apart from their own work? * Clarity of Presentation, the English does not need to be flawless, but the text should be understandable

The key strength of the paper is their novel approach to make a TTS system usable for ASR system training using very limited resources. The authors present a method to use only a single speaker from the target language to achieve improvements.

While this is a great achievement, the question remains how much the properties of this single speaker affect the results. It would be great to have included results by running the same experiment, but evaluating using speakers to assess to critical the choice of this one speaker is. Given such a scenario where only limited resources are available to utilize a single speaker, it may be crucial to select this speaker carefully to have the most impact.

As for the novelty, given the references the authors provide, other attempts have been made of using synthetic speech to train ASR systems (with a varying degree of success). However the setting the authors chose here introduces some novelty.

The experiments appear to be technically correct, however due to the double blind review process I could not (and did not attempt) to search for the paper #7 which contains more background information about the model used which would have been helpful for the assessment.

The references are adequate and provide a good overview of the related work.

The paper is sufficiently clear, except for the minor aspect mentioned above where paper #7 is unavailable. Assuming that this paper contains the few missing details about the system, there are no concerns about the clarity of the presentation.

Reviewer #5
Questions
1. Reviewer confidence (1-3) By selecting a value, you confirm that you are competent to evaluate this paper. If you have doubts about your ability to assess it, do not complete this form but instead use "Contact Meta-Reviewer". 
1: Sufficiently Confident
2. Technical correctness of the work (1-4) Please evaluate the scientific and/or technical correctness of the work. If experiments are presented please consider if enough details are provided on the datasets, baseline and experimental design to allow the experiments to be reproduced or equivalent experiments run. If you give a score of 1 or 2, please provide further explanation in your Detailed Comments.
2: Significant flaws that may call results into question
3. Clarity of presentation Please evaluate the clarity of the presentation of the work. Take into account the writing and quality of figures, tables etc. If you give a score of 1 or 2 please provide further explanation in your Detailed Comments.
3. Clear enough, could benefit from some revision
4. Overall recommendation (1-6)
4: Weak Accept: I am leaning to accept this paper
5. Detailed Comments for Authors Please supply detailed comments to back up your rankings. These comments will be forwarded to the authors of the paper. The comments will help the committee decide the outcome of the paper, and will help justify this decision for the authors. If the paper is accepted, the comments should guide the authors in making revisions for a final manuscript. Hence, the more detailed you make your comments, the more useful your review will be - both for the committee and for the authors. (min. 120 words). Particularly, provide feedback on the following topics: * Key Strength of the paper * Main Weakness of the paper * Novelty/Originality, taking into account the relevance of the work for the Interspeech audience * Technical Correctness, is the work technically and/or scientifically solid? Are sufficient details provided to allow any experiments to be reproduced or equivalent experiments run? * Quality of References, is it a good mix of older and newer papers? Do the authors show a good grasp of the current state of the literature? Do they also cite other papers apart from their own work? * Clarity of Presentation, the English does not need to be flawless, but the text should be understandable
In this paper, the authors propose data augmentation techniques for low-resource ASR using multi-speaker TTS and cross-lingual voice conversion. This is a relevant and interesting research topic.

Combining cross-lingual TTS and voice conversion seems a new direction of research. It is interesting to see that ASR can be improved in extremely low-resourced conditions in the target language.

Some critical pieces of information were missing in the submission:
1. In cross-lingual TTS, how were the linguistic units shared between the languages?
2. I understand the XyzTTS system had to be anonymized, but the basic details of the underlying technology have to be disclosed and are currently missing.
3. How does the XyzTTS system also perform voice conversion?

Other minor comments:
1. Portugese data: random sampling of utterances does not ensure that the test speakers are entirely different from those of the training. Have the authors ensured this?
2. "Although the focus of the model is on TTS it can also do zero-shot voice conversion" how is this possible?
3. "The explanation for "upper bound" is unclear.

Overall, if the above aspects are addressed, this work may be accepted for publication.



Reviewer #6
Questions
1. Reviewer confidence (1-3) By selecting a value, you confirm that you are competent to evaluate this paper. If you have doubts about your ability to assess it, do not complete this form but instead use "Contact Meta-Reviewer". 
2: Confident
2. Technical correctness of the work (1-4) Please evaluate the scientific and/or technical correctness of the work. If experiments are presented please consider if enough details are provided on the datasets, baseline and experimental design to allow the experiments to be reproduced or equivalent experiments run. If you give a score of 1 or 2, please provide further explanation in your Detailed Comments.
4: Technically solid
3. Clarity of presentation Please evaluate the clarity of the presentation of the work. Take into account the writing and quality of figures, tables etc. If you give a score of 1 or 2 please provide further explanation in your Detailed Comments.
3. Clear enough, could benefit from some revision
4. Overall recommendation (1-6)
5: Accept: I think this paper should be accepted
5. Detailed Comments for Authors Please supply detailed comments to back up your rankings. These comments will be forwarded to the authors of the paper. The comments will help the committee decide the outcome of the paper, and will help justify this decision for the authors. If the paper is accepted, the comments should guide the authors in making revisions for a final manuscript. Hence, the more detailed you make your comments, the more useful your review will be - both for the committee and for the authors. (min. 120 words). Particularly, provide feedback on the following topics: * Key Strength of the paper * Main Weakness of the paper * Novelty/Originality, taking into account the relevance of the work for the Interspeech audience * Technical Correctness, is the work technically and/or scientifically solid? Are sufficient details provided to allow any experiments to be reproduced or equivalent experiments run? * Quality of References, is it a good mix of older and newer papers? Do the authors show a good grasp of the current state of the literature? Do they also cite other papers apart from their own work? * Clarity of Presentation, the English does not need to be flawless, but the text should be understandable
The authors propose using TTS and voice conversion methods for training ASR models on low resource languages. In particular, they target a scenario where only a single speaker is available in the target language. For this purpose they train a TTS model with one high resource language (English) including multiple speakers (1248) and two low resource languages (pt_BR, ru_RU) trained on a single speaker.

From different ASR experiments they show that:
* When training the model with just synthesized speech but using the original target language audio for speaker embedding extraction, which is fed to the TTS model (thereby effectively using multiple speakers in the target language), the results are roughly 60% worse compared to training with the original audio.
* Adding audio augmentations such as noise addition, pitch shifting and RIR convolution improves the results for model trained with synthesized speech much more compared to that for the model trained with original audio. With augmentation, the relative performance gap is reduced to about 50-55%.
* When the TTS dataset uses just one target speaker to generate all training audio, the performance gap is larger compared to when the speaker embeddings are derived from the original audio.
* When the TTS datasets are generated by a combination of multi-speaker (where speaker embeddings are derived from english speakers) TTS and VC (trained on just one speaker in the target language) and augmented with original audio, WER reduces by 30-37% relative compared to using just the target audio.
* When the single speaker TTS dataset is augmented with multi-speaker TTS/VC dataset, the WER reduces by 50-55% compared to using just the single speaker TTS dataset.

Overall, the authors demonstrate that even if only one speaker is available in the target language, a reasonably accurate ASR model can be trained using a TTS/VC model trained from this speaker.

Key strength: The results are convincing, especially for the model trained with single speaker TTS + GEN_TTS + GEN_VC

Main weakness: The paper is mostly an application of the authors' previous work on training TTS model with a single speaker, which is used to train and compare different ASR models in this paper.

Novelty: The novelty here is mostly from the focus on the extreme low resource scenario with a strict assumption of only one speaker being available in the target language.

Technical correctness: The work is technically correct and provides sufficient details about the experimental results.

Quality of references: References are adequate.

Clarity of presentation: The technical description is sufficiently clear.
